Efficient Language Modeling with Sparse all-MLP

All-MLP architectures have attracted increasing interest as an alternative to attention-based models. In NLP, recent work like gMLP shows that all-MLPs can match Transformers in language modeling, but still lag behind in downstream tasks. In this work, we analyze the limitations of MLPs in expressiveness, and propose sparsely activated MLPs with mixture-of-experts (MoEs) in both feature and input (token) dimensions. Such sparse all-MLPs significantly increase model capacity and expressiveness while keeping the compute constant. We address critical challenges in incorporating conditional computation with two routing strategies. The proposed sparse all-MLP improves language modeling perplexity and obtains up to 2$\times$ improvement in training efficiency compared to both Transformer-based MoEs (GShard, Switch Transformer, Base Layers and HASH Layers) as well as dense Transformers and all-MLPs. Finally, we evaluate its zero-shot in-context learning performance on six downstream tasks, and find that it surpasses Transformer-based MoEs and dense Transformers.

==> content/5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}


In Fig.~\ref{fig:dense_comparison}, we compare our model with the dense model. The Transformer is the dominate dense mode, the other is the whole mlp model, which was published recently \citep{gmlp}. It can be seen from the figure that our model is better than dense Transformer and full mlp structure.


All the deep learning models in NLP are performing two major types of operations, one is token-wise operation, and the other is operations on hidden dimensions. For the Transformer \citep{vaswani2017attention} structure, it designs the self attention module for token-wise operation and FFN for hidden dimensions operation. For the gMLP \citep{gmlp} structure, it designs spatial linear layer for token-wise operation and FFN for hidden dimensions operation. For the previous MoE models \cite{gshard,switch,baselayer,hashlayer}, they use the standard self attention module for token-wise operation and sparse FFN for hidden dimensions operation. Our model is a full mlp sparse model, and the model structure is different from all of the previous models. For token-wise operation, we design a s-MoE layer; For hidden dimension operation, we choice the Base Layers \citep{baselayer} model. In the previous section, we mainly controlled the FLOPs of the model, and then compared the entire model. In this section, we will discuss three different token-wise operations: the self attention module, spatial linear module, and s-MoE module. 


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{iclr2022/img/compare_dense.png}
    \caption{Compared with dense model}
    \label{fig:dense_comparison}
\end{figure}

\begin{table*}[ht!]
    \centering
    \scalebox{1.0}{
    \begin{tabular}{l|c c c}
    \toprule
        Modules & heads & parameters & FLOPs \\
        \midrule
         self attention & 16 & 4.198 M & 12.885 G \\ 
         self attention & 1 & 4.198 M & 12.885 G \\ 
         spatial linear & 16 & - & -\\
         spatial linear & 1 & 1.054 M & 4.316 G\\
         s-MoE & 32 & 1.058 M & 2.147 G\\
         \bottomrule
    
    \end{tabular}}
    \caption{token-wise operations comparison.}
    \label{tab:token_wise}
\end{table*}

In Table~\ref{tab:token_wise}, we compare these three token-wise operations and their respective head mechanisms. The self attention module learns four weights $W_Q$, $W_K$, $W_V$ and output projection, where $W_Q, W_K, W_V \in \mathcal{R}^{head\ *\ hidden\_dim\ *\ hidden\_dim}$. When the self attention module increase the head number, it will reduce the the $hidden\_dim$ accordingly. Therefore, when increasing the heads number, the self attention module will keep the same parameters. In self attention, this multi-head mechanism greatly enhances the effect of the Transformer. 

As a comparison, the spatial linear module is 
\begin{equation*}
    \text{output} = W * \text{input}
\end{equation*}
, where $W \in \mathcal{R}^{head\ *\ seq\_len\ *\ seq\_len}$. At this time, once we increase the number of heads, the amount of parameters will greatly increase. At the same time, we found that in the mlp model, multi-head did not play a role.

Our sMoE-deterministic model assigns vectors to experts in a determinstic way. In this way, each head is equal to GPU number. When we increase head number, it will not increase the parameter number as well as FLOPs value. 


